Finite-sample analysis of M-estimators using self-concordance

The classical asymptotic theory for parametric $M$-estimators guarantees that, in the limit of infinite sample size, the excess risk has a chi-square type distribution, even in the misspecified case. We demonstrate how self-concordance of the loss allows to characterize the critical sample size sufficient to guarantee a chi-square type in-probability bound for the excess risk. Specifically, we consider two classes of losses: (i) self-concordant losses in the classical sense of Nesterov and Nemirovski, i.e., whose third derivative is uniformly bounded with the $3/2$ power of the second derivative; (ii) pseudo self-concordant losses, for which the power is removed. These classes contain losses corresponding to several generalized linear models, including the logistic loss and pseudo-Huber losses. Our basic result under minimal assumptions bounds the critical sample size by $O(d \cdot d_{\text{eff}}),$ where $d$ the parameter dimension and $d_{\text{eff}}$ the effective dimension that accounts for model misspecification. In contrast to the existing results, we only impose local assumptions that concern the population risk minimizer $\theta_*$. Namely, we assume that the calibrated design, i.e., design scaled by the square root of the second derivative of the loss, is subgaussian at $\theta_*$. Besides, for type-ii losses we require boundedness of a certain measure of curvature of the population risk at $\theta_*$.Our improved result bounds the critical sample size from above as $O(\max\{d_{\text{eff}}, d \log d\})$ under slightly stronger assumptions. Namely, the local assumptions must hold in the neighborhood of $\theta_*$ given by the Dikin ellipsoid of the population risk. Interestingly, we find that, for logistic regression with Gaussian design, there is no actual restriction of conditions: the subgaussian parameter and curvature measure remain near-constant over the Dikin ellipsoid. Finally, we extend some of these results to $\ell_1$-penalized estimators in high dimensions.

==> problem-statement-old.tex <==
%Consider the model of linear regression which in its simplest formulation can be summarized as follows.
Recall the standard setting of statistical learning: given a parametric set $\Theta \subseteq \R^d$ and a random observation $Z \in \Z$ with unknown distribution $\cP_*$, one would like to minimize the \textit{average risk}
\[
L(\theta) := \E_{*}[\ell_Z(\theta)],
\]
where for each possible value $z$ of $Z$, the \textit{loss} $\ell_{z}: \Theta \to \R$ specifies the price of choosing~$\theta$ provided that $Z = z$, and $\E_*[\cdot]$ is expectation with respect to the distribution~$\cP_*$ of $Z$. This distribution is assumed to be uknown, and the average risk cannot be computed and minimized directly. 
Instead, one is granted access to an i.i.d. sample~$Z_{1:n} = (Z_1, ..., Z_n) \in \mathcal{Z}^n$ with the same distribution as $Z$ (and independent of it), which is then used to construct an estimator $\wh\theta = \wh\theta(Z_{1:n})$ of the best value of the parameter, i.e.,
\[
\theta_* \in \Argmin_{\theta \in \Theta} L(\theta),
\]
under the assumption that such a value exists.
In particular, the sample gives rise to the \textit{empirical distribution}~$\mathscr{P}_n$ (the uniform probability measure supported on $Z_{1:n}$) and the \textit{empirical risk}
\[
L_n(\theta) := \frac{1}{n} \sum_{i=1}^n \ell_{Z_i}(\theta),
\]
an observable counterpart of $L(\theta)$. 
%the goal is to predict the response, given the design, as a linear combination of the latter with a \textit{predictor} $\theta \in \R^d$. 
%The prediction performance of a given value~$\theta$ is measured by the \textit{average risk} $L(\theta) := \E[\ell_{Z}(\theta)]$. 
Ideally, we would like to have an estimator with small \textit{excess risk}~$L(\wh\theta_n) - L(\theta_*)$ in probability, or at least, small \textit{average excess risk}~$\En[L(\wh\theta_n)] - L(\theta_*)$ where~$\En$ stands for the expectation over the sample $Z_{1:n}$. Since for each fixed value~$\theta$ of the parameter, $L_n(\theta)$ is an unbiased estimate of $L(\theta)$ which converges to $L(\theta)$ almost surely by the law of large numbers, a natural candidate estimator of $\theta_*$ is the \textit{empirical risk minimizer} (ERM):
\[
\wh\theta_n \in \Argmin_{\theta \in \Theta} L_n(\theta).
\]

%\paragraph{Quasi-MLE.}
Our main focus in this paper is the setting where $L_n(\theta)$ is a negative log-likelihood, meaning that $\ell_z(\theta) = \log p_\theta(z)$ where $p_\theta(\cdot)$ is some probability density supported on $\Z$\footnotemark.
\footnotetext{To include the case of discrete distributions, one can think of densities as Radon-Nikodym derivatives with respect to some dominating measure.}
In other words, one indirectly assumes that the sample is generated according to some distribution from the \textit{parametric family} $\Distrib = (\cP_\theta), \theta \in \Theta$, which may or may not contain the actual data-generating distribution $\cP_*$. When~$\cP_* \in \Distrib$, we say that the parametric model corresponding to $\Distrib$ is \textit{well-specified}; in this case, ERM becomes the maximum-likelihood estimator (MLE). 
Otherwise, the model is called \textit{misspecified}; ERM can then be regarded as \textit{quasi maximum-likelihood} estimator (q-MLE), sometimes also referred to MLE under \textit{model misspecification}. 
%Furthermore, in this latter case the average excess risk can be shown, under some regularity assumptions, to be exactly the Kullback-Leibler divergence between the actual data distribution $P$ and $P_\theta$.
In this case, $\cP_{\theta_*}$ corresponds to the ``projection'' of~$\cP_*$ onto the family $\Distrib$ in the sense of the Kullback-Leibler divergence, and q-MLE approximates $\cP_{\theta_*}$ by replacing $\cP_*$ with the observed empricial distribution~$\cP_n$ of the data.
Our work has been motivated by the following question:
\begin{align}
\label{Q}
\parbox{\dimexpr\linewidth-6em}{\textit{Can one extend the classical results on the local asymptotic normality of q-MLE \\ to the non-asymptotic setting?}}
\tag{\textit{Q}}
\end{align}
To clarify and substantiate~\eqref{Q}, it makes sense to briefly review the aforementioned results.
%$L(\theta) = \E\left[\frac{1}{2\sigma^2}\| y - x^\T \theta\|^2\right].$
%We will explain the meaning of $\sigma^2$ a bit later; for now, simply observe that all the bounds on the $L(\theta)$ must be rescaled by $2\sigma^2$ to obtain the familiar bounds for the conventionally defined quadratic risk.
%Here and in what follows, the norm without subscripts is the usual Euclidean one, and the expectation is taken with respect to the \textit{true} measure $P$ generating a new (testing) observation pair, unless explicitly stated overwise. 
%Given an i.i.d. sample $Z_{1:n} := (z_1, z_2, ..., z_n)$ with $z_i = (x_i, y_i) \sim P$  (so that $\Pn := P^{\otimes n}$ is the disrtibution of $S$), the empirical risk minimization (ERM) estimator $\wh \theta_n$ minimizes the \textit{empirical risk} $L_n(\theta)$:
%\[
%\wh\theta_n \in \Argmin_{\theta \in \R^d} \left\{ L_n(\theta) = \frac{1}{2\sigma^2n} \sum_{i=1}^n \| y_i - x_i^\T \theta \|^2 \right\}.
%\]
%Since for any given predictor $\theta$ one has $\E_S L_n(\theta) = L(\theta)$, one can hope that $\wh\theta_n$ will be a good estimate of the \textit{true minimizer} of the average risk, defined as
%\[
%\theta_* \in \Argmin_{\theta \in \R^d} L(\theta). 
%\]
%This intuition is quickly confirmed in the asymptotic setting as we show below.
%\paragraph{Local asymptotic normality.}
Most of them (see monographs~\cite{lehmann2006theory,ibragimov2013statistical,vdv,borovkov} among others) rely on the \textit{local regularity} assumptions about the log-likelihood, allowing for a second-order Taylor expansion of~$L(\theta)$ around~$\theta_*$.
In particular, it is assumed that $L(\theta)$ is sufficiently smooth at $\theta_*$, which is an internal point of~$\Theta$, so that the first-order optimality condition for $\theta_*$ reduces to $\nabla L(\theta_*) = 0$. 
Moreover, the Hessian 
\[
\He := \nabla^2 L(\theta_*)
\]
is assumed to be non-degenerate, i.e., $\He \succ 0$.
When combined together, these assumptions allow to derive the \textit{local asymptotic normality} of q-MLE: in the limit $n \to \infty$ with fixed~$d$, one has
% see, e.g.,~\cite{white1982maximum}
\begin{equation}
\label{eq:fisher}
\begin{aligned}
%\sqrt{n}(\wh\theta_n - \theta_*) &\dto \cN(0, \He^{-1} \Gr \He^{-1}),\\
\sqrt{n}\He^{1/2}(\wh\theta_n - \theta_*)  &\dto \cN(0, \He^{-1/2} \Gr \He^{-1/2}),
\end{aligned}
\end{equation}
where~$\Gr$ is the covariance matrix of the gradient of the loss at $\theta_*$:
\[
\Gr := \E_*[\nabla \ell_Z(\theta_*)\nabla \ell_{Z}(\theta_*)^\T].
\]
Matrices $\Gr$ and $\He$ remain fixed as $n$ grows, and hence the above results state, in particular, that the variance of~$\wh\theta_n - \theta_*$ decreases at the rate~$1/n$.
%and normalized matrix $\frac{1}{n}\Gamma$ is the covariance of the \textit{score} $\nabla L_n(\theta_*)$: 
%$
%\tfrac{1}{n}\Gr := \En [\nabla L_n(\theta_*)\nabla L_n(\theta_*)^\T]
%$
Moreover, in the well-specified case one has~$\Gr = \He,$ whence~$\sqrt{n} \He^{1/2}(\wh\theta_n - \theta_*) \dto \cN(0, \Id_d)$, known as \textit{Fisher's theorem}. 
Denoting~$\|\cdot\|_{\Ma}$ the seminorm related to the positive-semidefinite matrix $\Ma$ by $\|x\|_{\Ma}^2 = x^\T \Ma x$, we can see that 
\[
n\| \wh\theta_n-\theta_*\|_{\He}^2 \dto {\chi_d^2}
\] 
where $\chi_d^2$ is the chi-square law with $d$ degrees of freedom.
Finally, the local quadratic expansion of the average risk around $\theta_*$ allows to derive the same asymptotic law for the (scaled) average excess risk~$2n(L(\wh\theta_n) - L(\theta_*))$, the result known as \textit{Wilks' theorem}, implying, in particular, that
\[
\En[L(\wh\theta_n)]  - L(\theta_*) = \frac{d}{2n} + o(n^{-1}).
\] 
Moreover, the chi-square deviation bound, see~\cite[Lemma 1]{lama2000}, implies a bound in probability:
\begin{equation}
\label{eq:chi-square}
L(\wh\theta_n)  - L(\theta_*) = \frac{(\sqrt{d} + \sqrt{2\log(1/\delta)})^2}{2n} + o(n^{-1}).
\end{equation}
%where $c$ is some absolute constant. 
Finally, these $O(d/n)$ asymptotic bounds can be extended to the general situation of misspecified models. The extension of Fisher's theorem is 
ntroducing the \textit{effective dimension}:
\[
\deff := \E_* [\| \nabla\ell_Z(\theta_*) \|_{\He^{-1}}^2] = \tr (\He^{-1/2} \Gr  \He^{-1/2}).
\]
The expected excess risk bound then changes to
\begin{equation}
\label{eq:crb}
\En[L(\wh\theta_n)]  - L(\theta_*) = \frac{\deff}{2n} + o(n^{-1}),
\end{equation}
and the corresponding in-probability bound (see again~\cite[Lemma 1]{lama2000}) can be written as\footnotemark
\begin{equation}
\label{eq:crb-prob}
L(\wh\theta_n)  - L(\theta_*) = \frac{\deff (1 + \sqrt{2\log(1/\delta)})^2}{2n} + o(n^{-1}).
\end{equation}
In fact, the main term in the right-hand side of~\eqref{eq:crb} is the minimum possible asymptotic variance of any unbiased estimator; this result is known as the \textit{Cram\'er-Rao bound}. 
\footnotetext{Note that even with~$\deff = d$, there is still a difference between~\eqref{eq:crb-prob} and~\eqref{eq:chi-square}, the reason being that~\eqref{eq:crb-prob} corresponds to the ``generalied'' chi-square statistic~$\sum_{i=1}^d \sigma_i^2 \xi_i^2$ with i.i.d.~$\xi_i \sim \cN(0,1)$ and different $\sigma_i^2$, see \cite{lama2000}.}
For what is to follow, it is important to note that the asymptotic approach can be summarized in the following steps:
\begin{itemize}
\item[(i)]
First, the estimate is localized: $\|\wh\theta_n - \theta_*\|_{\He}^2$ is shown to behave as the squared ``natural'' norm of the score, $\|\nabla L_n(\theta_*)\|_{\He^{-1}}^2$, which is can be controlled by the central limit theorem.
\item[(ii)]
Using the second order Taylor expansion of $L(\theta)$ around $\theta_*$, similar behavior is obtained for the normalized excess risk~$2n[L(\wh\theta_n) - L(\theta_*)]$.
\end{itemize}


Despite its clarity and simplicity in use, the applicability of the classical theory is restricted by the necessity of taking the limit~$n \to \infty$ with fixed dimension of the parameter space. 
%hindering its application, especially in the context of high-dimensionality. 
% where $n$ and $d$ are comparable.
One approach towards the extension of the classical results, recently attempted in the literature, see~\cite{chernozhukov2014central,barbier2017phase}, allows for~$\deff \to \infty$ while requiring that the ratio~$\deff/n$ tends to a constant. However, this does not answer the outlined question~\eqref{Q}. 
%In contrast, here we are interested in obtaining \textit{finite-sample} analogues of the classical asymptotic consistency results. 
In contrast to that, the work~\cite{spokoiny2012parametric} outlined a general approach for extending the local asymptotic normality results to the setting of finite~$d$ and~$n$, partially answering~\eqref{Q}. 
The approach of~\cite{spokoiny2012parametric} can be described as follows.
The parameter space~$\Theta$ is divided into a certain elliptic neighborhood~$\Theta_*(r)$ of the true minimum and its complement.
Then, step (ii) of the asymptotic approach is replaced with so-called ``quadratic bracketing'': $L_n(\theta) - L_n(\theta_*)$ on~$\Theta_*(r)$ is bounded between two quadratic forms, each of them close to $\|\theta - \theta_*\|_{\He}$.
On the other hand, the ``localization'' step~(i) is replaced with the control of the event $\wh\theta_n \notin \Theta_*(r)$, by studying the uniform deviations of the empirical risk~$L_n(\theta) - L_n(\theta_*)$ using the advanced techniques from empirical process theory. 
This approach is quite powerful, allowing to derive the counterparts of the asymptotic results in the most challenging regime $n \ge C\deff$, the constant~$C$ only depending on the desired confidence. 
However, %its applicability is hindered
it is plagued by the strong \textit{global} assumptions on the pointwise deviations of the empirical risk process, which are necessary to control its uniform deviations (see Sections~2.2 and~4 in \cite{spokoiny2012parametric}).\\

In this paper, we propose a different approach towards answering~\eqref{Q}, inspired by, and partially rooted in, the work~\cite{hsu2016loss}. 

In fact, its applicability extends beyond the quasi-likelihood model to M-estimators with certain properties. 
%for the general quasi-MLE and Bayesian estimators, it can be addressed using the advanced machinery from the empirical processes theory, see, e.g.,~\cite{spokoiny2012parametric}. 
%Anyway, some sort of statistical threshold arises: the asymptotically optimal rate of convergence for ERM is established whenever the sample size is big enough in terms of the effective dimension. 
%In particular, the minimal sample size requirement arises in 
Namely, we focus on \textit{conditional linear prediction} models: the observations are given by~$Z = (X, Y)$, where \textit{response}~$Y$ is modeled as some function of the scalar product of~$\theta$ with random \textit{predictor}~$X \in \R^d$ whose distribution is not included in the parametric model.
In this case, $\ell_Z(\theta) = \ell(Y,X^\T\theta)$ for some function of two variables~$\ell(Y, \eta)$, and the Hessian of~$L(\theta)$ has the following structure:
\[
\nabla^2 L(\theta) = \E_* [\ell''(Y,X^\T \theta) \cdot XX^\T];
\]
hereinafter the derivatives of $\ell(Y,\eta)$ are with respect to the second variable. 
The Hessian~$\nabla^2 L(\theta)$ encapsulates the curvature information about the risk; in particular, $\nabla^2 L(\theta_*)$ defines the behavior of $L(\theta)$ close to its minimum. 
Meanwhile, the ERM estimator minimizes a noisy counterpart of $L(\theta)$, and only has access to the noisy estimate of the Hessian:
 \[
\nabla^2 L_n(\theta) =  \frac{1}{n} \sum_{i = 1}^n \ell''(Y_i,X_i^\T \theta) \cdot X_i X_i^\T.
\]
Hence, at least on an intuitive level, $\wh \theta_n$ should only be expected to be well-behaved when the sample size is large enough for the noisy Hessian~$\He_n := \nabla^2 L_n(\theta_*)$ to well-approximate its mean~$\He = \nabla^2 L(\theta_*)$, and possibly even only when this approximation is \textit{uniform} over some neighborhood of $\theta_*$ or the whole $\Theta$ -- which would appeal to the theory of empirical processes.
These challenges manifest already in the case of linear regression where the loss is quadratic, $\ell'' \equiv 1$, and hence the curvature properties of $L(\theta)$ are encapsulated in a single matrix~$\Var := \E[XX^\T]$. From the random matrix theory, it is known that as soon as~$n \gtrsim d$, the empirical second-moment matrix $\Varn := \frac{1}{n} \sum_{i=1}^n X_i X_i^\T$ provides a reliable estimate of $\Var$ in the sense that the semi-norm $\|\cdot\|_{\Varn}$ approximates the norm $\|\cdot\|_{\Var}$ up to a constant factor, see~\cite{vershynin2010introduction}. 
As we demonstrate below using a simple argument from~\cite{hsu2016loss}, this is sufficient to obtain finite-sample analogues of~\eqref{eq:crb}--\eqref{eq:crb-prob} in the setting of linear regression with random design.

\paragraph{Linear regression: asymptotic results.}
Let us define the residual $\varepsilon = Y - X^\T \theta_*$ where $\theta_*$ is the true minimizer of $L(\theta_*)$, and let $\sigma^2 = \E_*[\varepsilon^2]$; finally, let $\xi := \veps / \sigma$ be the normalized residual. 
We obtain a quasi-likelihood model corresponding to $Y \sim \cN(X^\T\theta_*,\sigma^2)$ taking $\ell$ to be the normalized square loss, 
\[
\ell(Y,X^\T\theta) = \frac{1}{2\sigma^2} (Y - X^\T\theta)^2,
\]
so that the MLE $\wh\theta_n$ is the ordinary least-squared estimator.
Let us first look at the asymptotic results in the present context. Whenever the model is well-specified, as a consequence of~\eqref{eq:crb} we obtain the $\frac{\sigma^2 d}{n}$ bound for the average excess risk of MLE:
\[
\En \E_* [(Y - X^\T \wh\theta_n)^2] - \sigma^2 = \frac{\sigma^2 d}{n}(1 + o(1)),
\]
and similarly for the bound in probability. More generally, under misspecification it holds
\[
\En \E_* [(Y - X^\T \wh\theta_n)^2] - \sigma^2 = \frac{\sigma^2 \deff}{n}(1 + o(1)). 
\]
It should be noted that in favorable circumstances one can bound $\deff$ in terms of $d$. 
Indeed,~$\nabla \ell_Z(\theta_*) = \xi X$ and~$\He = \frac{1}{\sigma^2}\Var$, whence 
\[
\deff = \E[\xi^2 \|\Var^{-1/2} X\|^2].
\]
Clearly, $\deff = d$ whenever $\xi$ and $x$ are independent, and $\xi$ is any distribution with $\E_*[\xi^2] = 1$.
More interestingly, under the finite fourth moment assumptions
\[
\sqrt{\E[\|\Var^{-1/2}X\|^4]} \le \kappa(X) \cdot \E[\|\Var^{-1/2}X\|^2], \quad
\sqrt{\E[Y^4|X=x]} \le \kappa(Y) \cdot \E[Y^2|X=x], \;\; \forall x \in \R^d,
\]
one has
\[
\deff \le \kappa(Y) \kappa(X) \cdot d
\] 
If the kurtoses\footnotemark~$\kappa(X), \kappa(Y)$ are bounded independently of $d$ and $n$ -- which is the case, for example, for subgaussian distributions of the data -- 
misspecified situation is not much more difficult than the well-specified one, at least with regards to the excess risk.
\footnotetext{Note that kurtosis is invariant under linear transforms, hence we can identify the kurtoses of $X$ and $\Var^{-1/2}X$.}


\paragraph{Linear regression: finite-sample results.} 
%Obtaining finite-sample analogues of the Cram\'er-Rao bound (CRB) is not straightforward in the case of random design, essentially due to the fact that the second-order information about the risk is noisy. 
Hsu and Sabato~\cite{hsu2016loss} suggested the following approach for obtaining $O({\sigma^2d}/{n})$ rate in linear regression with random design from the deviation bounds of empirical covariance matrices.
Assuming w.l.o.g. that $\sigma = 1$, the excess risk is simply a quadratic form:
\begin{equation}
\label{eq:ave-risk-linear}
L(\theta) - L(\theta_*) = \half \|\theta - \theta_* \|_\Var^2;
\end{equation}
correspondingly, the empirical excess risk is also a quadratic form: 
\begin{equation}
\label{eq:emp-risk-linear}
L_n(\theta)  - L_n(\theta_*) = \half \|\theta - \theta_* \|_\Varn^2 + \langle \nabla L_n(\theta_*), \theta-\theta_* \rangle,
\end{equation}
where $L_n(\theta_*)$ does not depend on $\theta$ so that $\nabla^2 L_n(\theta) \equiv \Var_n$. The key observation is that all global curvature information about $L(\theta)$ is encapsulated in a single matrix $\Var$, and we have an unbiased estimate $\Var_n$ of $\Var$ whose convergence to $\Var$ can be quantified non-asymptotically.
To be more specific, following~\cite{vershynin2010introduction}, let the subgaussian norm~$\|\zeta\|_{\psi_2}$ of a random variable $\zeta \in \R$ be
\[
\|\zeta\|_{\psi_2} := \inf \left\{b > 0 : \;\; \E [e^{\zeta^2/b^2}] \le 2 \right\},
\]
and more generally, for a random vector $Z \in \R^d$ let us define $\|Z\|_{\psi_2}$ as the maximal $\|\cdot\|_{\psi_2}$-norm of its one-dimensional marginals:
\begin{equation}
%\label{eq:subg-rd}
\|Z\|_{\psi_2} := \sup_{u \in \cS^{d-1}} \| \langle Z, u \rangle \|_{\psi_2},
\end{equation}
where $\cS^{d-1}$ is the unit sphere in $\R^d$. Assuming~$\E[X] = 0$, we have the following result, see~\cite{vershynin2010introduction}: %(see Appendix~\ref{app:cov-mat} for details):
\begin{theorem}[\cite{vershynin2010introduction}, Theorem 5.39]
\label{th:covariance-subgaussian-simple}
Assume that $X \in \R^d$ satisfies $\E[XX^\T] = \Var$ and 
$
\|\Var^{-1/2}X\|_{\psi_2} \le K.
$
Let $\Varn = \frac{1}{n} \sum_{i=1}^n X_i X_i^\T$ where $X_1, ..., X_n$ are independent copies of $X$. Whenever
\begin{equation}
\label{eq:cov-subgaussian-complexity}
n \gtrsim K^4 (d + \log(1/\delta)),
\end{equation}
with probability at least $1-\delta$ it holds
\begin{equation}
\label{eq:cov-dist-equiv}
\tfrac{1}{2} \|\theta\|^2_{\Var} \le \|\theta\|^2_{\Varn} \le 2 \|\theta\|^2_{\Var}, \quad \forall \theta \in \R^d.
\end{equation}
\end{theorem}
\begin{remark}
\textup{
A natural assumption is that~$K$ is a constant that does not depend on $(d, n, \delta)$. In particular, this holds for Gaussian design with arbitrary covariance matrix, as well as for subgaussian designs with squared $\psi_2$-norm comparable with the operator norm of the covariance~$\|\Var\|$, for example, when $\Var^{-1/2} X$ has independent components with Bernoulli distribution.
}\end{remark}

Following~\cite{hsu2016loss}, Theorem~\ref{th:covariance-subgaussian-simple} can be exploited as follows. 
%First, note that the empirical risk~$L_n(\theta)$ is $1$-strongly convex with respect to the norm $\|\cdot\|_{\Var_n}$ whenever~$\|\cdot\|_{\Var_n}$ is really a norm, cf.~\eqref{eq:cov-subgaussian-complexity}.
Whenever $n$ is such that~\eqref{eq:cov-subgaussian-complexity} is satisfied, due to~\eqref{eq:cov-dist-equiv} we have that
%Observe that $L_n(\theta)$ is $1$-strongly convex with respect to the norm $\|\cdot\|_{\Var}$, and is minimized in $\wh\theta_n$, whence
%$\half \|\wh\theta_n - \theta_* \|_{\Sigma_n}^2  L_n(\wh\theta_n) - L_n(\theta_*)$
with probability at least $1-\delta$, the norms $\|\cdot\|_{\Var}$ and~$\|\cdot\|_{\Varn}$ are within the factor~$2$ from each other, and~$L_n(\theta)$ is $\half$-strongly convex with respect to $\|\cdot\|_\Var$. 
Hence,
\[
\tfrac{1}{2} \|\wh\theta_n - \theta_* \|_{\Var}^2 \le \|\wh\theta_n - \theta_* \|_{\Varn}^2 \le \|\nabla L_n(\theta_*)\|_{\Var_n^{-1}}^2 \le 2\|\nabla L_n(\theta_*)\|_{\Var^{-1}}^2.
\]
Due to~\eqref{eq:ave-risk-linear}, this implies
$
L(\wh \theta_n) - L(\theta_*) = \half \|\wh\theta_n - \theta_* \|_{\Var}^2 \le 2\|\nabla L_n(\theta_*)\|_{\Var^{-1}}^2.
$
We managed to bound~$L(\wh \theta_n) - L(\theta_*)$ in terms of~$\|\nabla L_n(\theta_*)\|_{\Var^{-1}}^2$ with high probability, and we are essentially done: $\E[\|\nabla L_n(\theta_*)\|_{\Var^{-1}}^2] = \deff$, whence~\eqref{eq:crb-prob} follows if $Y$ is subgaussian\footnotemark. 
\footnotetext{
Otherwise, one can divide the sample into $\log(1/\delta)$ non-overlapping subsamples, compute independent least-squares estimators over this subsamples, and take as the final estimator their multi-dimensional median in the $\|\cdot\|_{\Varn}$-distance, see~\cite{hsu2016loss} for details.}
%\[
%2\|\nabla L_n(\theta_*)\|_{\Var^{-1}}^2
%\]
%  with respect to the norm $\|\cdot\|_\Var$, s. We also provide these computations in the appendix.
%%We obtained an analogue of~\eqref{eq:CRB-finite} in probability.
%\footnotetext{In fact, \cite{hsu2016loss} uses the matrix concentration result from~\cite{vershynin2010introduction} incorrectly, which results in an extra factor~$Q(\Var)$, the condition number of $\Var$, in~\eqref{eq:cov-subgaussian-complexity}. Our equivalent formulation of that result in Theorem~\ref{th:covariance-subgaussian-simple} concerns the \textit{standardized} design which allows to circumvent the issue.}

The main points of this argument can be summarized as follows: (i) for large enough $n$, the norm~$\|\cdot\|_{\Var_n}$ well-approximates the norm~$\|\cdot\|_{\Var}$, and~$L_n(\theta)$ is \textit{strongly convex}, with constant modulus, with respect to $\|\cdot\|_{\Var}$, which allows to bound $\tfrac{1}{2} \|\wh\theta_n - \theta_* \|_{\Var}^2$ in terms of~$\|\nabla L_n(\theta_*)\|_{\Var^{-1}}^2$; (ii) \textit{smoothness} of~$L(\theta)$, with modulus $\Omega(1)$, with respect to $\|\cdot\|_{\Var}$ allows to bound $L(\wh\theta_n) - L(\theta_*)$ in terms of $\half \|\wh\theta_n - \theta_* \|_{\Var}^2$ and hence~$\|\nabla L_n(\theta_*)\|_{\Var^{-1}}^2$.
%$\nabla L(\wh\theta_n)$, and then in terms of the score: $\nabla L_n(\theta_*)$ fluctuates around $\nabla L(\theta_*)$ which is close to $\nabla L(\wh\theta_n)$ if $L$ is smooth.
We are about to see how a similar argument can be conducted in a more general situation where the strong convexity and smoothness assumptions are not satisfied -- that of \textit{quasi self-concordant losses} in which one can control the precision of second-order Taylor approximation in terms of the Newton decrement (squared norm of the gradient in the norm of the inverse Hessian).
This generalization will bring in another statistical threshold in addition to~\eqref{eq:cov-subgaussian-complexity}: essentially, the sample size will be required to be large enough in order to guarantee that~$\|\nabla L_n(\theta_*)\|_{\Var^{-1}}^2$ is small enough.
%Interestingly, this can also be understood from the optimization standpoint. the Newton decrement to be small so that $\theta_*$ would be in the Dikin ellipsoid of~$\wh\theta_n$, see~\cite{nemirovski1994interior,nesterov2013introductory,bach2010self-concordant}.

\paragraph{Notation.}
Hereinafter, $f(\cdot) \lesssim g(\cdot)$ means that~$f(\cdot) \le Cg(\cdot)$ for some absolute constant~$C$. Symbol~$\dto$ denotes convergence in law. $[n]$ is the set of integers $\{1, 2, ..., n\}$.
Unless explicitly stated otherwise, $\wh\theta_n$ denotes the ERM estimator or its regularized version. Random vectors are denoted by capital letters (such as $Z$), and matrices by bold capital letters (such as $\Ma$). $\Id_d$ denotes the $d \times d$ identity matrix.
$\Ma^\T$ is the transpose of a matrix $\Ma$. For two semidefinite matrices $\Ma_1, \Ma_2$ of the same size, we write~$\Ma_1 \prccq \Ma_2$ whenever~$\Ma_2-\Ma_1$ is positive semidefinite. 
%$\|\cdot\|$ is the usual $\ell_2$-norm when the argument is a vector or an element of a Hilbert space. 
We use the $\ell_p$-norms $\|\cdot\|_p$ in $\R^d$ or in a Hilbert space (in the latter case the norm is assumed to be finite for the argument of interest).
The same notation is used for the Schatten norms of matrices and, more generally, operators in a Hilbert space: $\|\Ma\|_2$ is the Frobenius norm and $\|\Ma\|_\infty$ is the sup-norm (a.k.a. the operator norm).
Finally, given a matrix~$\Ma \succq 0$, we define the Mahalanobis norm~$\|\theta\|_{\Ma} := \|\Ma^{1/2} \theta \|$.

==> qsc-properties-old.tex <==
\subsection{Properties of (pseudo) self-concordant functions}
\label{sec:qsc-properties}
Here we summarize technical results about quasi-self-concordant functions that we will exploit. 
Fix two arbitrary parameter values $\theta_0, \theta_1 \in \Theta$, and consider functions~$\phi(\cdot)$,  $\phi_n(\cdot)$ on $\R$ defined by 
\begin{equation}
\label{def:line-restriction}
\begin{aligned}
%\phi_Z(t) = \ell_Z(\theta_t), \quad 
&\phi(t) = L(\theta_t), \quad \phi_{n}(t) = L_n(\theta_t)\\
&\text{where} \;\; \theta_t := \theta_0 + t(\theta_1-\theta_0), \; t \in [0,1].
\end{aligned}
\end{equation}
We first state a straightforward consequence of Assumptions~\ref{ass:basic}, \ref{ass:gsc-true}, and~\ref{ass:gsc-fake} for these functions. Its proof is a routine application of the chain derivative rule, and hence is omitted.
%of the link for $L_n(\theta)$ and $L(\theta)$. 
%This notation allows to avoid working with the tensor of third derivatives of $\ell_Z(\theta)$.
%Note that due to the GLM structure, one has the following identities:
%\begin{align}
%&\nabla \ell_z(\theta) = \xi x, \quad \xi = a'(x^\T\theta)-y,\\
%&\nabla^2 \ell_z(\theta) = a''(x^\T\theta) \cdot xx^\T, \\
%&\nabla^2 L_n(\theta) = \frac{1}{n} \sum_{i=1}^n a''(x_i^\T\theta) \cdot x_i x_i^\T, \\
%&\nabla^2 L(\theta) = \E [a''(x^\T\theta) \cdot x x^\T].
%\end{align}
\begin{proposition}
\label{prop:line-gsc}
%\thmlinebreak
%Consider function $\phi: \R \to \R$ given by 
%\[
%\phi(t) = \alpha^\T \theta_t + \beta + \frac{1}{n} \sum_{i=1}^n a(x_i^\T \theta_t), \quad \theta_t = \theta_0 + t(\theta_1-\theta_0),
%\] 
%for some $x, \theta_0, \theta_1 \in \R^d$, where $\alpha$ and $\beta$ do not depend on $\theta$, and assume that $a(\eta)$ satisfies~\eqref{ass:gsc} with some $\nu \in [1, 3/2]$.
%Then for any $t \in \R$ one has
%\[
%\phi^{(p)}(t) = \frac{1}{n} \sum_{i=1}^n (\langle x_i, \theta_1-\theta_0 \rangle)^p \cdot a^{(p)}(x_i^\T \theta_t), \quad p \in \{2,3\},
%\]
%whence
\begin{itemize}
\item[(a).]
Suppose that the loss satisfies Assumptions~\ref{ass:basic} and~\ref{ass:gsc-true}, then
\begin{align}
\label{eq:line-gsc-true-n}
&|\phi'''_n(t)| \le 2[\phi''_n(t)]^{3/2},\\ 
\label{eq:line-gsc-true-ave}
&|\phi'''(t)| \le 2[\phi''(t)]^{3/2}. 
\end{align}
\item[(b).] Suppose that instead of Assumption~\ref{ass:gsc-true}, one has Assumption~\ref{ass:gsc-fake} satisfied, then
\begin{align}
\label{eq:line-gsc-fake-n}
&|\phi'''_n(t)| \le \phi''_n(t) \cdot \max_{i \in [n]} |\langle X_i, \theta_1-\theta_0 \rangle| .
\end{align}
 %$S_X = |\langle X, \theta_1-\theta_0 \rangle|$,~\
Moreover, whenever the supremum below exists, one has
\begin{align}
\label{eq:line-gsc-fake-ave}
&|\phi'''(t)| \le \phi''(t) \cdot \sup_{x \in \X} |\langle X, \theta_1-\theta_0 \rangle|.
\end{align}
\end{itemize}
\end{proposition}
%Note that~$S_X$, $S_n$ and~$S$ disappear from the right-hand sides of~\eqref{eq:line-gsc-Z}--\eqref{eq:line-gsc-ave} in the case~$\mu = \frac{3}{2}$.

%\begin{proposition}
%Suppose that $\phi(t): \R \to \R$ satisfies a scaled counterpart of~\eqref{ass:gsc}: $\phi \in C^3(\R)$ and
%\[
%|\phi'''(t)| \le r\phi''(t).
%\]
%Then, the following is true: 
%\end{proposition}

The next two propositions summarize the local properties of self-concordant functions, and describe their behavior close to the optimum. 
Their parts corresponding to Assumption~\ref{ass:gsc-true} have been proved in~\cite[Sections 4.1.4--4.1.5]{nemirovski1994interior}, 
while those corresponding to Assumption~\ref{ass:gsc-fake} subsume~\cite[Propositions 1--2]{bach2010self-concordant}.

\begin{proposition}%[Proposition 1 in~\cite{bach2010self-concordant}]
\label{prop:local}
Let $F(\cdot)$ be a convex $C^3$ mapping $F: \Theta \to \R$, and let $\phi_F(t) := F(\theta_t)$.
Denote~$\He_0 = \nabla^2 F(\theta_0) \prccq 0$, $\He_1 = \nabla^2 F(\theta_1)$, and~$r = \|\theta_1 - \theta_0\|_{\He_0}$. 
\begin{itemize}
\item[(a).]
If~$\phi_F(t)$ satisfies
$
|\phi'''_F(t)| \le 2[\phi''_F(t)]^{3/2}
$
for any $\theta_1 \in \Theta$, one has the following approximations:
%let~$S \le R \|\theta_1-\theta_0\|_{\Ma}$ for , and let~
\begin{align}
\label{eq:local-upper-true}
{F(\theta_1) - F(\theta_0) - \nabla F(\theta_0)^\T (\theta_1-\theta_0)} &\le -r - \log(1-r),\\
\label{eq:local-lower-true}
{F(\theta_1) - F(\theta_0) - \nabla F(\theta_0)^\T (\theta_1-\theta_0)} &\ge r - \log(1+r),
\end{align}
%\begin{equation}
%\label{eq:hessian-true}
%(1-r)^2 \cdot \He_0 \prccq \He_1 \prccq (1-r)^{-2} \cdot \He_0,
%\end{equation}
where~\eqref{eq:local-upper-true} %and~\eqref{eq:hessian-true} 
holds whenever~$r < 1$.

\item[(b).] 
If~$\phi_F(t)$ satisfies, instead, 
$
|\phi'''_F(t)| \le R \|\theta_1-\theta_0\|_{\He_0} \cdot \phi''_F(t)
$
for some $R \ge 0$, and denoting 
\[
\tau := R r,
\]
one has
\begin{align}
\label{eq:local-upper-fake}
{F(\theta_1) - F(\theta_0) - \nabla F(\theta_0)^\T (\theta_1-\theta_0)} &\le \left(\frac{e^{\tau}-\tau-1}{\tau^2}\right) \cdot r^2,\\
\label{eq:local-lower-fake}
{F(\theta_1) - F(\theta_0) - \nabla F(\theta_0)^\T (\theta_1-\theta_0)} &\ge \left(\frac{e^{-\tau}+\tau-1}{\tau^2}\right) \cdot r^2.
\end{align}
%\begin{equation}
%\label{eq:hessian-fake}
%e^{-S} \cdot \He_0 \prccq \He_1 \prccq e^{S} \cdot \He_0.
%\end{equation}
\end{itemize}

\end{proposition}

%\begin{remark}
%\textup{
%Similar approximations in terms of $r$, with factors converging to a constant as $u_1 - u_0 \to 0$, can be derived for other ``homogeneities'' of self-concordance, arising from functions satisfying $|\phi'''(t)| \le [\phi''(t)]^{\nu}$ for some $\nu \ge 1$, see also a recent preprint \cite{sun2017generalized}.
%In particular, this allows to address the classical self-concordance in the sense of Nesterov and Nemirovski~\cite{nemirovski1994interior}, relevant in the context of logarithmic link function which arises in canonical exponential families for convex bodies~\cite{bubeck2014entropic}.
%}\end{remark}

%The next proposition describes the behavior of self-concordant functions close to the optimum. It subsumes~\cite[Sections 4.1.4--4.1.5]{nesterov2013introductory} and~\cite[Proposition 2]{bach2010self-concordant}.

\begin{proposition}
\label{prop:dikin}
Let $F$ be as in the premise of Proposition~\ref{prop:local}, and suppose that~$\He_0 \succ 0$. %where $\lambda[\cdot]$ denotes the lowest eigenvalue of a positive semi-definite matrix.

\begin{itemize}
\item[-]
In case (a): whenever
\[
\|\nabla F(\theta_0) \|_{\He_0^{-1}}^2 \le \tfrac{1}{4},
\]
then~$F(\theta)$ has a unique global minimizer $\tilde \theta \in \Theta$, and 
$
\|\tilde \theta - \theta_0\|_{\He_0}^2 \le 4  \| \nabla F(\theta_0) \|_{\He_0^{-1}}^2.
$
\item[-]
In case (b): whenever
\[
{R^2 \| \nabla F(\theta_0) \|_{\He_0^{-1}}^2} \le \tfrac{1}{4},
\]
then~$F(\theta)$ has a unique global minimizer $\tilde \theta \in \Theta$, and 
$
\|\tilde \theta - \theta_0\|_{\He_0}^2 \le 16 \| \nabla F(\theta_0) \|_{\He_0^{-1}}^2.
$
\end{itemize}
\end{proposition}
The key feature of the above proposition is that \textit{local} information about~$F(\cdot)$ at \textit{one point} in fact provides \textit{global} information about the proximity of this point to the optimum of~$F(\cdot)$.
%Let us now apply these tools to GLMs with link functions satisfying~\eqref{ass:gsc}. 

==> ridge.tex <==
\subsection{Tikhonov regularization}
\label{sec:ridge}
In this section, we address the non-parametric setting where the set~$\Theta$ is replaced with a Hilbert space~$\cH$ with norm~$\|\cdot\|_{\cH}$ which can be identified with $\ell\|\cdot\|_2$ in some orthonormal basis. 
For simplicity, we assume that optimization is now unconstrained).
As such, the dimensions $d$ and~$\deff$ can now be infinite, and the sample complexity bounds established in Section~\ref{sec:main-results} become meaningless. Instead, we consider the $\ell_2$-penalized estimator 
\[
\wh\theta_n^{\lambda} \in \Argmin_{\theta} L_n(\theta) + \frac{\lambda}{2} \| \theta\|_2^2,
\]
%and compare it with the best estimator of the penalized risk:~$\theta_*^{\lambda} \in \Argmin_{\theta}  L(\theta) + \lambda \| \theta\|_2^2.$
Note that~$\theta_*^{\lambda}$ is itself an approximation of the true risk minimizer~$\theta_*$, since $L(\theta_*^{\lambda}) -  L(\theta_*) \ge 0$. 
In the case of linear regression, the error~$L(\theta_*^{\lambda}) -  L(\theta_*)$ corresponds to the deterministic bias, and can be expressed as

\paragraph{Approximation error.}

We first quantify the proximity of~$\theta_*$ to the solution of the penalized problem 
\[
\theta_\lambda \in \Argmin_{\theta} L(\theta) + \frac{\lambda}{2} \| \theta\|_2^2.
\] 
We have the following proposition.
\begin{proposition}
\label{prop:l2-bias}
Assume~\ref{ass:gsc-fake} and~\ref{ass:curvature}. 
Let $\He_\lambda := \He + \lambda \Id$, $\Cov_{\lambda} = \Cov + \lambda \Id$, and for~$\bar R_\lambda(X) \ge 0$,
\[
\|\Cov_\lambda^{-1/2}X\|_2 \le \bar R_\lambda(X), \;\; \text{$\cP$-a.s}.
\]
Moreover, let~$\lambda$ be chosen such that 
\[
\bb_1 := \lambda^2 \|\He_\lambda^{-1/2} \theta_*\|^2 \le \frac{1}{4\rho \bar R_\lambda^2(X)}.
\]
Then, 
\begin{equation}
\label{eq:l2-bias-fake}
L(\theta_\lambda) - L(\theta_*) \lsim \|\theta_* - \theta_\lambda\|_{\He_{\lambda}}^2 \lsim \bb_1.
\end{equation}
\end{proposition}

\begin{proof}
Consider function~$L_{\lambda}(\theta) := L(\theta) + \frac{\lambda}{2} \|\theta\|_2^2$ which is minimized at $\theta_\lambda$, so that~$\nabla L_{\lambda}(\theta_\lambda) = 0$. 
Note that 
\[
\nabla L_\lambda(\theta_*) = \lambda \theta_*, \quad 
\nabla^2 L_\lambda(\theta_*) = \He_{\lambda}.
\]
Clearly, $L_{\lambda}(\theta)$ satisfies case~\ref{prop:local-bach} of Proposition~\ref{prop:local} at~$\theta_*$ with $R^2 = \rho \bar R^2_\lambda(X)$, where we used that
\[
\|X\|_{\He_{\lambda}^{-1}}^2 \le \|\Cov_{\lambda} \He_{\lambda}^{-1}\|_{\infty} \bar R^2_\lambda(X)  \le \|\Cov \He^{-1}\|_{\infty} \bar R^2_\lambda(X) \le \rho \bar R^2_\lambda(X).
\]
%since it is a sum of $L(\theta)$ that satisfies this proposition, and a quadratic function. 
Hence, by Proposition~\ref{prop:dikin}, we get that whenever~$\bb_1 = \lambda^2 \|   \theta_* \|_{\He_\lambda^{-1}}^2 \le \rho \bar R_\lambda^2(X)/4,$
we have that
\[
\|\theta_* - \theta_\lambda\|_{\He_{\lambda}}^2 \lsim \bb_1.
\]
On the other hand, consider function~$Q_{\lambda}(\theta) := L(\theta) + \frac{\lambda}{2} \|\theta_{\lambda} - \theta_*\|_2^2$ that also satisfies case~\ref{prop:local-bach} of Proposition~\ref{prop:local}. 
Note that~$\nabla^2 Q_\lambda(\theta_*) = \He_{\lambda}$, and~$\nabla Q_{\lambda}(\theta_*) = 0$. Applying~\eqref{eq:local-upper-fake} with~$\theta_0 = \theta_*$ and~$\theta_1 = \theta_\lambda$, and proceeding as in part~$\boldsymbol{2}^o$ of the proof of Theorem~\ref{th:crb-fake-simple}, we get 
\[
Q_{\lambda}(\theta_\lambda) - Q_{\lambda}(\theta_*) \lsim  \|\theta_* - \theta_\lambda\|_{\He_{\lambda}}^2.
\]
The left inequality~\eqref{eq:bias-fake} then follows since~$L(\theta_\lambda) - L(\theta_*) \le Q_{\lambda}(\theta_\lambda) - Q_{\lambda}(\theta_*)$. 
\end{proof}

\paragraph{Stochastic error.}
We now show a counterpart result for the stochastic error $L(\wh\theta_n) - L(\theta_\lambda)$. 
\begin{proposition}
\label{prop:l2-variance}
\end{proposition}
